Safety Verification of Model Based Reinforcement Learning Controllers

Model-based reinforcement learning (RL) has emerged as a promising tool for developing controllers for real world systems (e.g., robotics, autonomous driving, etc.). However, real systems often have constraints imposed on their state space which must be satisfied to ensure the safety of the system and its environment. Developing a verification tool for RL algorithms is challenging because the non-linear structure of neural networks impedes analytical verification of such models or controllers. To this end, we present a novel safety verification framework for model-based RL controllers using reachable set analysis. The proposed frame-work can efficiently handle models and controllers which are represented using neural networks. Additionally, if a controller fails to satisfy the safety constraints in general, the proposed framework can also be used to identify the subset of initial states from which the controller can be safely executed.

==> methodology.tex <==
\section{Safety Verification}
In this section, we first present the problem setting and specify the assumptions made in this work, followed by the proposed algorithm.
%

\subsection{Model-Based Reinforcement Learning}


%%%%%%%%%%%%%%%%
\subsection{Reachable Set Analysis}
In this section we give a brief overview of the HJI PDE formulation required to compute the BRT for a non-linear system with uncertain parameters.

Before formally defining a BRT, we introduce the problem setting.
%
The goal is to determine the set of states which can reach a target set $\mathcal{L} \subset \mathbb{R}^n$ under finite time.
%
While computing the BRT, convention is that the target set is reached at final time $t_f = 0$ and the finite time trajectory starts at some initial time $t_0 = -T, \; 0 < T < \infty$. 
%
The system follows the dynamics $f(s, a)$ and its initial states are represented as $\mathcal{S}_0 \in \mathcal{S}$. % where $s \in \mathcal{S} \subset \mathbb{R}^n$ is the state space and $a \in \mathcal{A} \subset \mathbb{R}^m$ is the action space.
%
%The control policy $\pi: \mathcal{S} \rightarrow \mathcal{A}$ determines the action to take in any state $s$ and thus, drives the system either towards or away from the target set.
%
Additionally, there might be a disturbance in the system or the environment which affects the system state as well.
%
This disturbance is represented using a finite set $\mathcal{D} \subset \mathbb{R}^n$ and is considered as a control input which can affect the progression of the system states in an undesired manner. 
%
Let $f_r: \mathcal{S} \times \mathcal{A} \times \mathcal{D} \rightarrow \mathcal{S}$ denote the augmented system dynamics which also takes into account the disturbance input $d \in \mathcal{D}$ to determine the next state.
%
\begin{assumption}
The control inputs $a$ and $d$ are drawn from closed and bounded sets, i.e., finite sets $\mathcal{A} \subset \mathbb{R}^m$ and $\mathcal{D} \subset \mathbb{R}^m$ respectively.
\end{assumption}
%
Besides the assumptions made in this work, we explicitly state the assumptions from \cite{TheHolyOne, mitchell2005time} as requirements for Theorem \ref{thm1} stated below and later prove how our assumptions fulfill these requirements to leverage the results from previous works.
%
\begin{reqm} \label{req1}
The system  dynamics $f_r(s, a, d)$ is uniformly continuous, bounded and Lipschitz continuous in $s$ while the inputs $a$ and $d$ are fixed.
\end{reqm}

\begin{reqm} \label{req2}
The target set $\mathcal{L} \subset \mathbb{R}^n$ is closed and can be represented as the zero sublevel set of a bounded and Lipschitz continuous function $l: \mathbb{R}^n \rightarrow \mathbb{R}$ as
\begin{equation}
    \mathcal{L} = \{ s: l(s) \le 0\}.
    \label{eqn:target_level_func}
\end{equation}
\end{reqm}
%
Thus, (\ref{eqn:target_level_func}) determines a way to check whether a state lies inside or outside the target set $\mathcal{L}$.
%
If $\mathcal{L}$ can be represented using a regular, well-defined geometric shape (like a sphere, rectangle, cylinder etc.) then deriving the level set function $l(s)$ is straight forward.
%
An irregularly shaped $\mathcal{L}$ can be represented as a union of several well-defined geometric shapes to derive $l(s)$.
%
%The following reachability formulation is developed for an unsafe target set $\mathcal{L}$, i.e., the optimal policy $\pi(s)$ is developed to avoid the target set.

From the above information, we formally define the BRT for a finite time $T$, $R_B(T)$ as the set of states that can reach $\mathcal{L}$ within time $T$, despite the disturbance $d$ in the system.
%
Specifically, if $\mathcal{L}$ is an unsafe target set, we are interested in determining the subset of initial states $\mathcal{S}_{unsafe} \subset \mathcal{S}_0$ such that for all trajectories starting from an initial state $s_0 \in \mathcal{S}_{unsafe}$ there exists a sequence of actions $a(\cdot)$ which will eventually drive the system following dynamics $f_r(s, a, d)$ to $\mathcal{L}$ despite the disturbance.
\begin{equation}
\begin{split}
    R_B(T) := \{ s_0: \exists a, \; s.t. &\; \forall d, \; s(\cdot) \; satisfies \; \dot{s}=f_r(s,a, d), \\
    s(0)=s_0; &\; \exists t \in [-T, 0], \; s.t. \; s(t) \in \mathcal{L} \}
    \end{split}
    \label{eqn:backward_reach_dist}
\end{equation}

The above goal of computing $R_B(T)$ can be achieved by formulating the BRT as an optimal control problem.
%
From (\ref{eqn:target_level_func}), a trajectory is said to reach $\mathcal{L}$ if it's state at the final time step $t_f = 0$ satisfies $l(s(0)) \le 0$.
%
Similarly, if $l(s(0)) > 0$ then the trajectory never reaches $\mathcal{L}$.
%
Therefore, to formulate the BRT problem as an optimal control problem a function $\phi$ is defined as
\begin{equation}
\begin{split}
    \phi(s(t), t) &= \max_a \min_d l(s(0)), \; t \in [-T, 0] \\
    \text{s.t. } \; \; \dot{s} &= f_r(s, a, d) \\
    l&(s(0)) \le 0
\end{split}
\label{eqn:game_opt}
\end{equation}
where the control input $a \in \mathcal{A}$ is driving the system away from the unsafe target set $\mathcal{L}$ by maximizing the value of $l(s(0))$ at the final time step and the disturbance control is doing the opposite.
%
The above formulation is a 2 player game where player 1 is the controller and player 2 is the disturbance.
%
The choice of formulating the problem as a maximin optimization gives the advantage to player 2 \cite{TheHolyOne}, thereby ensuring that a worst case scenario is considered for player 1 and the BRT is over approximated to give a conservative solution.
%
It should be noted that depending on whether the target set is safe or unsafe, the optimization formulation in (\ref{eqn:game_opt}) can be modified according to the table \ref{tab:game_opt}.
\begin{table}
\begin{center}
\caption{Optimization objectives of players for safe and unsafe target sets.} \label{tab:game_opt}
\begin{tabular}{| c | c | c | }
  \hline
  & Unsafe target set & Safe target set \\ 
  \hline
 Player 1 & max $\phi$ & min $\phi$ \\  
 \hline
 Player 2 & min $\phi$ & max $\phi$ \\  
 \hline
\end{tabular}
\end{center}
\end{table}
%
\begin{reqm} \label{ass3}
The input signals are drawn from the following sets
\begin{equation}
    \begin{split}
        a(\cdot) \in \mathcal{A}(t) \overset{\Delta}{=} \{ \eta:[-T, \; 0] \rightarrow \mathcal{A}| \eta(\cdot) \text{ is measurable} \}\\
        d(\cdot) \in \mathcal{D}(t) \overset{\Delta}{=} \{ \eta:[-T, \; 0] \rightarrow \mathcal{D}| \eta(\cdot) \text{ is measurable} \}
    \end{split}
\end{equation}
where $\mathcal{A} \subset \mathbb{R}^m$ and $\mathcal{D} \subset \mathbb{R}^m$ are compact and $T > 0$.
\end{reqm}

We now state theorem 3 from \cite{TheHolyOne} or equivalently theorem 2 from \cite{mitchell2005time} because it is essential to validating the algorithm proposed in the next section.

\begin{theorem} \label{thm1} Under requirements 1-3, let $\phi: \mathbb{R}^n \times [-T, \; 0] \rightarrow \mathbb{R}$ be the viscosity solution of the terminal value HJI PDE
\begin{equation}
\begin{split}
    D_t \phi(s, t) + \min[0, H(s, \; D_s \phi(s, t))] &= 0, \\
    \phi(s, 0) &= l(s) \\
\text{where,} \; H(s, p) &= \max_{a \in \mathcal{A}} \min_{d \in \mathcal{D}} p^T f_r(s, a, d).
\end{split}
\label{eqn:PDE_HJI}
\end{equation}
Then, the zero sublevel set of $\phi$ describes $B_R(t)$
\begin{equation}
    B_R(t) = \{s \in \mathbb{R}^n | \phi(s, t) \le 0 \}.
\label{eqn:BRT}
\end{equation}
\end{theorem}
\begin{proof} See proof of theorem 3 in \cite{TheHolyOne} or theorem 2 in \cite{mitchell2005time}.
\end{proof}

%The viscosity solution ensures that under suitable conditions $\phi$ remains bounded and continuous for all times.
%
The formulation in (\ref{eqn:PDE_HJI}) is key to computing the BRT and a numerical solution for $\phi$ using the level set methods gives an implicit representation of $B_R(t)$ in (\ref{eqn:BRT}).
%
%The implementation is discussed in details in Section \ref{sec:implementation}.

\textbf{Forward Reachable Set (FRS):}
The HJI formulation can also be used to compute the forward reachable set by forming an initial value PDE.
%
Using the same notation defined above, the FRS is defined as all the states which can be reached from an initial set $\mathcal{L}$ in finite time $T, \; 0< T < \infty$ despite the disturbance $d$.
%
\begin{equation}
\begin{split}
F_R(T) := \{s: \exists a, \text{ s.t. } \forall d, s(\cdot) \text{ satisfies } \dot{s} = f_r(s, a, d), \\
s(0) \in \mathcal{L}; s(T) = s \}
\end{split}
\end{equation}

Using a change of variables the terminal value PDE in (\ref{eqn:PDE_HJI}) can be converted into an initial value PDE and solved for the FRS.
%
The FRS has been used to analyze the output range of an ANN controller and can be used to determine whether or not a policy $\pi$ is safe for a given set of initial states $\mathcal{L}$.
%
\begin{equation}
    F_R(T) \cap \mathcal{C}_s = \begin{cases} = \emptyset
    &\mbox{if } \pi \text{ is safe} \\
    \neq \emptyset &\mbox{if } \pi \text{ is not safe} \end{cases}
\end{equation}
%
However, the FRS can only give a binary answer regarding the safety of the policy.
%
But by computing the BRS, we provide the set of initial states for which a given policy $\pi$ is safe.
%
Thus, by computing the BRS we can make a stronger statement regarding the policy.

\section{Methodology}
\label{sec:methodology}
%
This section presents the proposed algorithm and details the mathematical formulation required to compute the BRT for a general non-linear model of the learnt system dynamics.
%
\subsection{Overview}
The goal of the proposed algorithm is to verify the safety (i.e. constraint satisfaction) property of the given controller $\pi(s)$ by solving problem \ref{prob1}.
%
For given initial states $\mathcal{S}_0$ a policy $\pi(s)$ can be classified as either completely safe, completely unsafe or partially safe.
%
$\pi(s)$ is said to be completely safe if all the initial states are safe states and is said to be completely unsafe if none of the initial states are safe.
%
Mathematically, this can be verified by the following set operations
%
\begin{equation}
\mathcal{S}_{safe} \cap \mathcal{S}_0 = \begin{cases} \emptyset 
    & \implies \pi(s) \mbox{ is completely unsafe} \\
      \mathcal{S}_0
    & \implies \pi(s) \mbox{ is completely safe.}
\end{cases}
\label{eqn:safe_policy}
\end{equation}
%
The third case is the most interesting one where there is a subset of states for which $\pi(s)$ is safe, i.e., $\mathcal{S}_{safe} \subset \mathcal{S}_0$ and hence it is classified as a partially safe policy.

Thus, to classify a policy we need to determine $\mathcal{S}_{safe}$.
%
In the proposed algorithm this is achieved by computing the BRT from the constrained region $\mathcal{C}_s$ to first determine the subset of unsafe states $\mathcal{S}_{unsafe} \subset \mathcal{S}_0$, followed by using simple set operations to determine $\mathcal{S}_{safe}$.
%
The formulation in (\ref{eqn:PDE_HJI}) is used to compute the BRT.
%
However, the true system dynamics is unknown and only data tuples $D$ observed from the environment are known.
%
Therefore, the learnt model $\hat{f}(s, a)$ will be used to construct the BRT.

Since the learnt model is imperfect, we first determine the modelling error to bound the error uncertainty in the model.
%
By analyzing the prediction error of the learnt model $\hat{f}(s, a)$ over the validating data set $D_v$, we identify certain properties (like mean error) to determine the error bounds on the model as $\underline{d} < d < \overline{d}$.
%
Subsequently, this error bound is used to construct the augmented model $\hat{f}_r(s, a, d)$ which is used to compute the BRT.
%
To achieve this, the modification in the mathematical formulation in (\ref{eqn:PDE_HJI}) is presented in the next subsection.
%
Once the BRT is computed, it's intersection with the set of initial states $\mathcal{S}_0$ is used to get the desired solution to problem $\ref{prob2}$.
%
The overview is given in algorithm \ref{algo2}.

\begin{algorithm}
\label{algo2}
 \caption{Safety verification of model-based RL policy (INCOMPLETE)}
%\SetAlgoLined
%\begin{algorithmic}[1]
\KwInput{$\pi, \hat{f}(s, a), \mathcal{C}_s, \mathcal{S}_0$}
 $[ \underline{d}, \; \overline{d}] \leftarrow EstimateModellingError(\hat{f}(s, a), D_v)$\;
 $B_C(-T) \leftarrow BRT(\hat{f}(s, a, d), \pi(s), \mathcal{C}_s)$\;
 $\mathcal{S}_{unsafe} \leftarrow B_C(-T) \cap \mathcal{S}_0$\;
 $\mathcal{S}_{safe} = \overline{\mathcal{S}}_{unsafe} \cap \mathcal{S}_0$
\end{algorithm}

\subsection{Proposed Algorithm}
The proposed algorithm is divided in 3 steps:
%\begin{framed}
% \begin{itemize}[itemindent=2em]
  \paragraph{Step 1: \textit{Determining modelling error}}
  
  Recall that the model-based controller $\pi(s)$ and the learnt model $\hat{f}(s, a)$ are already known.
  %
  The first task is to determine the augmented system dynamics $\hat{f}_r(s, a, d)$ where the disturbance input $d \in \mathcal{D} \subset \mathbb{R}^n$ represents the modelling error.
  %
  Using the additive formulation in (\ref{eqn:model_error}) the augmented system dynamics is represented as
  \begin{equation}
      \hat{f}_r(s, a, d) = \hat{f}(s, a) + d.
      \label{eqn:aug_dynamics}
  \end{equation}
  %
  To determine the bounds on the modelling error, the feedforward pass in (\ref{eqn:feedforward}) is conducted over the validation data set $D_v$ for the learnt model $\hat{f}(s, a)$ and the squared error between the predicted state and the desired state values is computed.
  %
  This squared error is computed separately for each of the $n$ output states of the learnt model and for all the data points in the validation set.
  %
  Analyzing the individual state prediction errors for every data point in $D_v$ gives metrics like the mean, variance, s.d. etc. to estimate the bounds of the modelling error such that $\underline{d} < d < \overline{d}$.
  %
  The exact choice of the metric depends on the problem setting and how conservative a bound is required. 
  
  \paragraph{Step 2: \textit{Determine BRT for unsafe sets}}
  
  Instead of directly computing the set of safe initial states $\mathcal{S}_{safe}$ required in problem 1, a complementary problem is framed below.
  
  \begin{problem} \label{prob2}
  For a given unsafe set $\mathcal{C}_s$ determine the subset of unsafe initial states $\mathcal{S}_{unsafe} \subset \mathcal{S}_0$ such that for any initial state $s_0 \in \mathcal{S}_{unsafe}$ there exists at least one trajectory $\tau$ which will reach $\mathcal{C}_s$ under finite time while following the policy $\pi(s)$ under the disturbance $d$.
  \end{problem}
  
  To determine $\mathcal{S}_{unsafe}$ in problem \ref{prob2} the BRT from the unsafe target set $\mathcal{C}_s$ is constructed using (\ref{eqn:PDE_HJI}) and it is denoted as $B_{\mathcal{C}}(T)$.
  %
  Then $\mathcal{S}_{unsafe} = B_{\mathcal{C}}(T) \cap \mathcal{S}_0$.
  
  Since the true system dynamics is unknown, the formulation in (\ref{eqn:PDE_HJI}) has to be modified to substitute the system dynamics $f_r(s, a, d)$ with the learnt dynamics in (\ref{eqn:aug_dynamics}).
  %
  Additionally, the control input $a$ is now determined by the policy $\pi(s)$.
  %
  These changes are incorporated in the formulation (\ref{eqn:PDE_HJI}).
  
  The overall HJI PDE formulation remains the same, however the maximin Hamiltonian is modified to a constrained problem as
  \begin{equation}
\begin{split}
    H_{const}(s, p) &= \max_{a \in \mathcal{A}} \min_{d \in \mathcal{D}} p^T \hat{f}_r(s, a, d) \\
    \text{s.t. } &a = \pi(s) 
\end{split}
\label{eqn:HJI_appx_con}
\end{equation}
Since the action $a$ is computed by the deterministic policy $\pi(s)$, the outer maximization optimization is carried over a singleton set thereby simplifying (\ref{eqn:HJI_appx_con}) to 
% 
\begin{equation}
    H_{const}(s, p) = \min_{d \in \mathcal{D}} p^T [ \hat{f}(s, \pi(s)) + d ]
\end{equation}
%
where the modelled dynamics from (\ref{eqn:aug_dynamics}) are substituted above.
%
It is observed that the vector product $p^T \hat{f}(s, \pi(s))$ is independent of the design variable $d$ and can be taken out of the optimization.
\begin{equation}
    H_{const}(s, p) = p^T \hat{f}(s, \pi(s)) \; + \; \min_{d \in \mathcal{D}} p^T d 
    \label{eqn:H_opt1}
\end{equation}
%
Further, it is possible to derive an analytical solution of (\ref{eqn:H_opt1}).
%
By expanding the objective function $\min_{d \in \mathcal{D}} p^T d = \min_{d \in \mathcal{D}} (p_1 d_1 + p_2 d_2 + \hdots + p_n d_n)$ it is evident that depending on the sign of the costate terms, an optimal minimizing disturbance input can be computed as 
\begin{equation}
d_i = \begin{cases} -d_i
    &\mbox{if } p_i > 0 \\
      d_i
    &\mbox{if } p_i < 0 \end{cases} , \forall i=1,\hdots n,
\label{eqn:H_opt2}
\end{equation}
%
The analytical solution is therefore given as
\begin{equation}
\begin{split}
    H_{const}(s, p) = p^T \hat{f}(s, &\pi(s))  \\
    - &(|p_1| d_1 + |p_2| d_2 + \hdots + |p_n| d_n). 
    \end{split}
    \label{eqn:H_opt2}
\end{equation}

We are now ready to present the modified BRT problem formulation as
\begin{equation}
\begin{split}
    D_t \phi(s,t) + \min[0, H_{const}(s, \; D_x \phi(s,t))] &= 0, \\
    \phi(s, 0) &= l(s) \\
\text{where, } H_{const}(s, p) = p^T \hat{f}(s, \pi(s)&) \\
- (|p_1| d_1 + |p_2| d_2 +& \hdots + |p_n| d_n)
\end{split}
\label{eqn:PDE_HJI_v2}
\end{equation}
  
  \begin{theorem}
  Let $\phi$ be the viscosity solution of the terminal valued PDE in (\ref{eqn:PDE_HJI_v2}), then the zero sublevel set of $\phi$ describes the backward reachable set $B_C(t)$ as
  \begin{equation}
      B_C(t) = \{ s \in \mathbb{R}^n | \phi(s, t) \le 0\}.
      \label{eqn:thm_main}
  \end{equation}
  \label{thm:main}
  \end{theorem}
  %
  \begin{proof}
  For the proof of Theorem \ref{thm:main}, we leverage the result from Theorem \ref{thm1}.
  %
  To do so, we first ensure that our formulation satisfies the necessary requirements for Theorem \ref{thm1} to hold:
  %
 \paragraph{For Requirement 1 } From assumptions \ref{ass1} and \ref{ass2} it has been shown that an ANN modelled dynamics satisfies the properties of boundedness, uniform continuity and Lipschitz continuity for a large choice of activation functions. Therefore, the learnt dynamics $\hat{f}(s, a, d)$ satisfies requirement 1.
 %
 \paragraph{For Requirement 2 } From the discussion in Section \ref{sec:prelim}-C, a bounded and Lipschitz continuous function $l$ can easily be derived for a bounded target set $\mathcal{L}$ by representing it as a union of several well-defined geometric shapes. Therefore, for bounded constrained regions $\mathcal{C}_s$ this requirement is also satisfied.
%  
 \paragraph{For Requirement 3 } Finally, from assumption \ref{ass3} it is established that the input sets $\mathcal{A}, \mathcal{D} \subset \mathbb{R}^m$ are compact sets.
  
  Since our formulation satisfies all the necessary requirements of Theorem 1, the result of Theorem \ref{thm:main} follows directly from it.
  %
  Therefore, by computing the constrained Hamiltonian $H_{const}$ and solving for the viscosity solution $\phi$ in (\ref{eqn:PDE_HJI_v2}), the backward reachable set at any time $t$ is implicitly defined using (\ref{eqn:thm_main}).
  \end{proof}
  \paragraph{Step 3: \textit{Determine $\mathcal{S}_{safe}$}}
  
  In the final step, $\mathcal{S}_{safe}$ is determined from the solution of problem \ref{prob2}.
  %
  From the definitions of $\mathcal{S}_{safe}$ and $\mathcal{S}_{unsafe}$ in problem \ref{prob1} and \ref{prob2} respectively the following two statements are evident.
  %
  \begin{equation}
  \begin{split}
    \mathcal{S}_{safe} \cup \mathcal{S}_{unsafe} &= \mathcal{S}_0\\
    \mathcal{S}_{safe} \cap \mathcal{S}_{unsafe} &= \emptyset
    \end{split}
    \label{eqn:set_int}
  \end{equation}
  Therefore, it follows
  \begin{equation}
    \mathcal{S}_{safe} = \overline{\mathcal{S}}_{unsafe} \cap \mathcal{S}_0.
  \end{equation}
% \end{itemize}
%\end{framed}

After determining $\mathcal{S}_{safe}$ the policy can be classified as either completely safe, completely unsafe or partially safe by checking the conditions in (\ref{eqn:safe_policy}).
%
%We follow the methodology by a short note on the implementation of the algorithm.

\begin{comment}
\subsection{Algorithm Overview}
The proposed algorithm solves problem 1 in two steps.
%
In step 1 a complementary problem is solved to determine $\mathcal{S}_{unsafe}$ and in step 2 the solution from  problem 2 is used to determine $\mathcal{S}_{safe}$.

\textit{Step 1:}
Instead of directly computing $\mathcal{S}_{safe}$, a complementary problem is framed as follows:
\textbf{Problem 2:}
For given unsafe set $\mathcal{C}_s$ determine the unsafe subset of initial states $\mathcal{S}_{unsafe} \subset \mathcal{S}_0$ such that for any initial state $s_0 \in \mathcal{S}_{unsafe}$ there exists at least one trajectory $\tau$ under deterministic policy $\pi(s)$ which will drive the system state to $\mathcal{C}_s$ within a finite time.

To determine $\mathcal{S}_{unsafe}$ in problem 2, the backward reachable tube $B_R(T)$ from $\mathcal{C}_s$ is computed using (\ref{eqn:PDE_HJI}).
%
Then $\mathcal{S}_{unsafe} = B_R(T) \cap \mathcal{S}_0$.
%
The mathematical formulation is given in the following subsection.

\textit{Step 2:}
In this step, $\mathcal{S}_{safe}$ is determined from the solution of problem 2.
%
From the definitions of $\mathcal{S}_{safe}$ and $\mathcal{S}_{unsafe}$ in problem 1 and 2 respectively the following two statements are evident.
%
  \begin{equation}
  \begin{split}
    \mathcal{S}_{safe} \cup \mathcal{S}_{unsafe} &= \mathcal{S}_0\\
    \mathcal{S}_{safe} \cap \mathcal{S}_{unsafe} &= \emptyset
    \end{split}
    \label{eqn:set_int}
  \end{equation}
Therefore, it follows
\begin{equation}
    \mathcal{S}_{safe} = \overline{\mathcal{S}}_{unsafe} \cap \mathcal{S}_0.
\end{equation}


\subsection{Mathematical Formulation}
Since the actual system dynamics is unknown and only a learnt model $\hat{f}(s, a)$ is available, we first determine the bounds on the modelling error $d \in \mathcal{D} \subset \mathbb{R}^n$.
%
The bounds are determined for each state in the $n$-dimensional input vector such that $d_{min} < d < d_{max}$.
%
From the formulation in (\ref{eqn:model_error}) the two player system dynamics can be represented as
\begin{equation}
    \hat{f}(s, a, d) = \hat{f}(s, a) + d.
    \label{eqn:dyn_ad}
\end{equation}
%
The HJI PDE formulation remains the same however the hamiltonian is modified as follows:
\begin{equation}
\begin{split}
    H_{const}(s, p) &= \max_{a \in \mathcal{A}} \min_{d \in \mathcal{D}} p^T \hat{f}(s, a, d) \\
    \text{s.t. } &a = \pi(s) 
\end{split}
\label{eqn:HJI_appx_con}
\end{equation}
Since the action $a$ is computed by the deterministic policy $\pi(s)$, the outer maximization optimization is carried over a singleton set thereby simplifying (\ref{eqn:HJI_appx_con}) to 
% 
\begin{equation}
    H_{const}(s, p) = \min_{d \in \mathcal{D}} p^T [ \hat{f}(s, \pi(s)) + d ]
\end{equation}
%
where the modelled dynamics from (\ref{eqn:dyn_ad}) are substituted above.
%
It is observed that the vector product $p^T \hat{f}(s, \pi(s))$ is independent of the design variable $d$ and can be taken out of the optimization.
\begin{equation}
    H_{const}(s, p) = p^T \hat{f}(s, \pi(s)) \; \min_{d \in \mathcal{D}} p^T d 
    \label{eqn:H_opt1}
\end{equation}
%
Further, it is possible to derive an analytical solution of (\ref{eqn:H_opt1}) by expanding the objective function $p^T d$ as 
\begin{equation}
    H_{const}(s, p) = p^T \hat{f}(s, \pi(s)) \; \min_{d \in \mathcal{D}} (p_1 d_1 + p_2 d_2 + \hdots + p_n d_n). 
    \label{eqn:H_opt2}
\end{equation}
%
The analytical solution is therefore given as
\begin{equation}
    H_{const}(s, p) = p^T \hat{f}(s, \pi(s))  - (|p_1| d_1 + |p_2| d_2 + \hdots + |p_n| d_n). 
    \label{eqn:H_opt3}
\end{equation}

We are now ready to present the modified backward reachable tube problem formulation as
\begin{equation}
\begin{split}
    \frac{\partial J}{\partial t} + \min[0, H_{const}(s, \; \frac{\partial J}{\partial s})] &= 0, \\
    J(s, 0) &= l(s) \\
\text{where,} \; H_{const}(s, p) = p^T \hat{f}(s, \pi(s)) &- (|p_1| d_1 + |p_2| d_2 + \hdots + |p_n| d_n)
\end{split}
\label{eqn:PDE_HJI_v2}
\end{equation}

\end{comment}

